Performance modelling of access control mechanisms for local and vehicular wireless networks

Carrier sense multiple access collision avoidance (CSMA/CA) is the basic scheme upon which access to the shared medium is regulated in many wireless networks. With CSMA/CA a station willing to start a transmission has first to find the channel free for a given duration otherwise it will go into \emph{backoff}, i.e. refraining for transmitting for a randomly chosen delay. Performance analysis of a wireless network employing CSMA/CA regulation is not an easy task: except for simple network configuration analytical solution of key performance indicators (KPI) cannot be obtained hence one has to resort to formal modelling tools. In this paper we present a performance modelling study targeting different kind of CSMA/CA based wireless networks, namely: the IEEE 802.11 Wireless Local Area Networks (WLANs) and the 802.11p Vehicular Ad Hoc Networks (VANETs), which extends 802.11 with priorities over packets. The modelling framework we introduce allows for considering: i) an arbitrarily large number of stations, ii) different traffic conditions (saturated/non-saturated), iii) different hypothesis concerning the shared channel (ideal/non-ideal). We apply statistical model checking to assess KPIs of different network configurations.

==> sectionsCR/measurements.tex <==
\subsection{Measurement settings}
\label{sec:measures}
We have designed experiments aimed at assessing the performances of the network model in different respects. Specifically we  have assessed the impact of: 1) a faulty channel, 2) the incoming traffic,   3) the network dimension (i.e. the number of stations in the network) and 4) the packet size on the network performances. The results presented below have been all obtained through experiments executed with \prism\ \emph{statistical engine}, with the following settings: a $99\%$ confidence level and a fixed sample size of a 1000 paths. We stress that, because of the prohibitive  complexity of the network model  (which would result in a huge space state for the corresponding DTMC), using the statistical engine of \prism\ was the only realistic option. 

\paragraph{Nominal maximum busyTimeRatio.} We observe that the busyTimeRatio (BTR) of a network whose stations use the  RTS/CTS MAC scheme is upper bounded by a \emph{nominal maximum}  which corresponds with an ideal (hypothetical) situation where a continuos flow of DATA packet are transmitted without inter-arrival delay and in absence of collisions. In such situation the BTR is given by the ratio  of  busy-time over total-time for successfully  transmitting, where the latter (in absence of collisions) is straightforwardly obtained by considering the   \texttt{DIFS}-RTS-\texttt{SIFS}-CTS-\texttt{SIFS}-DATA-\texttt{SIFS}-ACK sequence, that is: 
\begin{equation}
\label{eq:nmbtr}
NominalMaxBTR = TXtime/ (SENSEtime+TXtime)
\end{equation}
where $TXtime\!=\!RTS\!+\!CTS\!+\!DATA\!+\!ACK$, is the total transmission time and $SENSEtime\!=\!\texttt{DIFS}\!+\!3\texttt{SIFS}$ is the total carrier-sensing time. From parameters in Table~\ref{tab:timeparams}, we have that $NominalMaxBTR\!=\!80/88\!=\! 0.909$, meaning that the optimal channel utilisation for a WiFi based on RTS/CTS 802.11 MAC cannot trespass $\sim\!90\%$. In the remainder we will see that  the BTR measures obtained through \prism\ exhibit  indeed an asymptotic  profile towards $NominalMaxBTR$. 



%\paragraph{Impact of incoming traffic.} Figure~\ref{fig:exptraffic}\\

\paragraph{Impact of network dimension and incoming traffic.} Figure~\ref{fig:impactNetDim} depicts results of experiments aimed at assessing the impact of the network dimension (num. of stations) on the performance and under the ideal channel hypothesis. Specifically  Figure~\ref{fig:impactNetDim}(a) (resp. Figure~\ref{fig:impactNetDim}(b)), displays the network throughput (resp. BTR) obtained by assessing formula $\psi_1$ (resp.  $\psi_2$)  in function of the incoming traffic rate ($\lambda$) in a non-saturated network and considering  networks of different   dimensions.  As expected both the throughput and  the BTR,  exhibits an asymptotic profile (the faster the inter-arrival rate the higher the throughput, resp. the  BTR) which is upper bounded by the throughput under saturated regime (which is $\sim\! 640$ packets per second), resp. the saturated nominal maximum BTR~(\ref{eq:nmbtr}).\\

%\paragraph{Impact of packet sizel.} Figure~\ref{fig:exptraffic}\\


\noindent
Results presented in Figure~\ref{fig:impactNetDim} refer to the \emph{ideal channel} setting of the model, meaning that a packet being transmitted has virtually zero probability of being dropped because of an error affecting the channel\footnote{We used  \texttt{mediumErrorSpikeFrequency}=200, i.e. prob. the channel enters burst-error state is $p=10^{-200}$}. 

\paragraph{Impact of faulty channel.} Figure~\ref{fig:expfaultychan} illustrates results of experiments aimed at assessing the effect that a faulty channel has on the network performances.  The  network throughput measured  in function of the \texttt{mediumErrorSpikeFrequency}  parameter (i.e. in function of the  probability the channel enters a burst-error phase, see Table~\ref{tab:chanerrorparams}) is given in Figure~\ref{fig:expfaultychan}(a), showing that the throughput increases as the probability of the channel's  burst error  decreases, however it is unaffected by the network  dimension (identical plot for different number of stations) indicating that the performances gradient induced by the network dimension in case of ideal channel (Figure~\ref{fig:impactNetDim}) fades away in presence of a faulty channel. The remaining settings for these experiments are: saturated traffic, \texttt{mediumErrorSpikeLength}=3 and a 50\% chance that an error actually occurs ( \texttt{mediumErrorRateWhileSpike}=0.5) when the channel is in  burst-error phase.    


%\begin{figure*}
%\begin{center}
%%\hfill
%\subfigure[saturated traffic]{\includegraphics[scale=.25]{PIC/throughputVspikeErrornStations}}
%\hskip 3ex
%\subfigure[\small 2 stations, non-saturated traffic]{\includegraphics[scale=.25]{PIC/throughputVspikeErrornStations_diffLamda}}
%\label{fig:BTR}
%\hfill
%\caption{Impact of faulty channel on a network performances}
%\label{fig:expfaultychan}
%\end{center}
%\end{figure*}
\noindent
Conversely Figure~\ref{fig:expfaultychan}(b) shows that  the burst error probability has different effects on the throughput  a non-saturated  network of fixed dimension (i.e. 5 stations) depending of the traffic arrival rates. 

\paragraph{Other measurements.} Apart from the throughput and BTR measures we developed  a number of other performance indicators which we also assessed against  different configurations of the model. Examples of such farther measures are the {\bf Average forwarding turnaround time} (i.e. average time needed to forward a packet from a source  station to a target station), and {\bf Average backoff round at transmission} (i.e. the average number of collisions occurred to successfully transmit a packet from source to destination). For the sake of space we refrain from presenting these results here. 



==> sectionsCR/modelling_80211.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Performance analysis of 802.11 DCF through the PRISM model checker}
\section{Performance modelling of 802.11 MAC}% with PRISM } %PRISM model checker}
\label{sec:prismperfanalysis}
%To   analyse the performances of the RTS/CTS version of the 802.11 DCF   we have developed a family of DTMC models under  the \prism\  framework.  %%Each model of the family which are suitable for  different scenarios (different type of traffic, ideal/error-prone channels
%Such models depends on many parameters 
%Each model of the family %is based  on the assumptions given below and 
%represents a network with  a specific number $N$ of stations and is generated through a Python script starting from a minimal  network with $N=2$  stations. 
%Each such \prism\ template  encode   the  802.11 DCF RTS/CTS double handshaking mechanism while taking into account different channel scenarios  (perfect/imperfect channel hypothesis).  \\
%Each model is based on the following modelling assumptions. 
Using the \prism\ model checker we have developed a (parametric) DTMC  model suitable for representing a network consisting of an arbitrary number $N$ of  stations that communicate using the 802.11 RTS/CTS DCF\footnote{we developed a  (in \texttt{Python}) script that based on a \emph{minimal network} DTMC model of a network with $N=2$  stations, generates the \prism\ model for a network with arbitrary $N$ stations, available for download \url{https://sites.google.com/site/pballarini/models}.}.  %An instance of such model refers to a network consisting of a specific number of nodes. For \prism\ DTMC models we have also developed a script (in \texttt{Python}) that starting from the minimal model of a network with $N=2$  stations, generates the corresponding model for a network with arbitrary $N$ stations. The python script as well as the minimal \prism\ DTMC model are available for download\footnote{\url{https://sites.google.com/site/pballarini/models}}.

\subsection{Modelling assumptions}
%\paragraph{Modelling assumptions.} 
The \prism\ DTMC  model we developed relies on the following assumptions: 
\begin{itemize}
%\item there are $N$ stations in the network
\item {\bf Clicque network topology}: the network consists of $N$  stations arranged in  a clique (i.e.  every station can overhear every other station).  
\item {\bf Traffic direction}: each station  has a unique target station to which it addresses   all its incoming traffic. 
\item {\bf Incoming traffic}: the incoming traffic of each station is supposed to obey  either 1) a \emph{saturated  regime} (i.e. a packet ready to be transmitted is invariably present) or  2) an arrival  Poisson process with parameter $\lambda$. The type of considered incoming traffic can be chosen through a specific parameter of the model. 
\item {\bf Perfect/Imperfect channel}: the wireless medium  is supposed to behave either 1) as a \emph{perfect channel} (i.e. transmitted  data are never  affected by errors) or  2) as an \emph{imperfect channel} with some error probability (details below). % in Section~\ref{sec:bursterrmodel}). %below for details of the type of errors the model account for). 
\item {\bf RTS/CTS protocol}:  stations use the 802.11 RTS/CTS DCF  scheme to access the medium. 
\item {\bf Vulnerable period}:  the radio device of each station is supposed to exhibit a certain delay for switching between transmission/reception mode. The duration of such period is called the \emph{vulnerable period} and is one source  of traffic collisions within the network.  
\end{itemize}

\paragraph{Channel error.} 
\label{sec:bursterrmodel}
To model the possibility that transmissions undergo errors due to the channel we adopted the burst-noise binary channel model~\cite{Gilbert60}. 
A noisy binary channel   is seen as a process that on receiving of a sequence of binary input digits $x_i$  adds a sequence of randomly generated noise digits $z_i$ to produce the output signal $y_i=x_i+z_i$. Although  the  generation of noisy digits may be  \emph{memoryless} (i.e. \emph{symmetric} binary channels), in practice  channels (in particular  radio channels)  exhibit memory,  hence errors tend to group in bursts (i.e. burst-noisy channel). 
%Within a burst-noisy channel then, errors are assumed to occur  in bursts rather than in single, independent occurrences.
Burst noise channels may be modelled through a two-states DTMC (Figure~\ref{fig:burstnoisedtmc}) as follows: state $G$ (good) represents the absence of noise digits, whereas  $B$ (burst errors) is a macro-state (consisting of states $B_{\hat{e}}$ and $B_{e}$) whereby bursts of noise digits may occur, i.e. a  noise digit is generated with probability $h$ (typically $h=0.5$). 
\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=.18]{PIC/noiseburstDTMC_v2}
\caption{A 2-states DTMC model of a burst-noise channel}
\label{fig:burstnoisedtmc}
\end{center}
\end{figure}
The burst behaviour is reproduced by letting  the  probability of a  transitions between $G$ and $B$  , i.e. $P[X_{n+1}\!=\!B | X_n\!=\!G]=p$ and $P[X_{n+1}\!=\!G | X_n\!=\!B]=p'$ (where $X_n$ is the state of the DTMC at time $n$),  considerable low (i.e. $p\ll q$, $p'\ll q'$, with $q\!=\! 1\!-\!p$ and $q'\!=\! 1\!-\!p'$). 
\noindent
Inner state  $B_{e}$ (resp. $B_{\bar{e}}$) is the state which is entered whenever  a noise digit is (resp. is not)  generated during an error burst period. 

%%%%%% TABLE CHANNEL-ERROR PARAMETERS %%%%%%%%%%
%\begin{table*}[htp]
%\scriptsize
%\begin{center}
%\begin{tabular}{|c|C{3cm}|c|}
%\hline
% \multicolumn{3}{|c|}{channel burst-error  parameters}\\
%\hline
%\hline
%name & meaning & definition/value \\
%\hline
%%&&\\
%$p$ & prob.  channel enters  burst-error & $10^{-mediumErrorSpikeFrequency }$\\
%$p'$  & prob.  channel exits  burst-error & $\frac{1}{mediumErrorSpikeLength\!+\! 1}$\\
%\texttt{mediumErrorSpikeFrequency} &  independent variable for determining  & variable\\
%&  the prob. of entering the burst-error   & \\
%\texttt{mediumErrorSpikeLength} & independent variable for determining  & variable\\
%&  the prob. of exiting the burst-error   & \\
%\texttt{mediumErrorRateWhileSpike} ($h$) & prob. of channel error  & 0.5 \\ 
%& while in burst error state &\\
%\hline
%\hline
% \multicolumn{3}{|c|}{input traffic parameters}\\
%\hline
%name & meaning & definition/value \\
%\hline
%\texttt{aSlotDurationInSeconds}   &  duration in sec of a time-slot & $10^{-5 }$\\
%\texttt{lambda}    & traffic arrival  rate  (Poisson) & variable \\
%\texttt{p1} &  prob. of an arrival in next time-slot  & $e^{-\texttt{lambda}\cdot\texttt{aSlotDurationInSeconds}}$\\
%\hline
%\end{tabular}
%\end{center}
%\caption{Burst-error and input traffic parameters of Prism  DTMC  network model}% : first measurements}
%\label{tab:chanerrorparams}
%\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Following the notion of burst noise channel we have integrated the two-state burst-noise  DTMC behaviour  within our \prism\ models of the 802.11 DCF. 
Specifically we have equipped the \texttt{Channel} module of \prism\  (see file \texttt{rtscts.pm} available at \url{}), which models the actual transmission of data through the radio channel,  with transitions representing the entering/exiting  into an error-burst state in which, an ongoing transmission can become \emph{garbled}  at each (discretised) \emph{slot} of time (i.e. $slotTime$) 


%%%% UPPAAL TIME-AUTOMATON FOR RTS/CTS SENDING STATION %%%%
%\begin{figure*}[htbp]
%\begin{center}
%%\includegraphics[scale=0.4,angle=90]{PIC/StationUppaal}
%\includegraphics[scale=0.6]{PIC/stationTemplate}
%\caption{Template timed-automaton  of a station using RTS/CTS DCF}
%\label{fig:stationTA}
%\end{center}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Input traffic.}
\label{sec:trafficmodel}
To analyse the effect that different traffic conditions have on the network performances we modelled the input traffic at each station as a Poisson process with rate $\lambda\!\in\!\mathbb{R}_{\geq 0}$, hence we assumed  that the inter-arrival time of incoming data follows a negative   exponential distribution of  rate $\lambda$, i.e. $Exp(\lambda)$. However since our models are DTMC (hence time is inherently discrete)  we have adopted a geometric  approximation of the negative exponential distribution. Specifically  given that a time unit in our DTMC model of 802.11 DCF corresponds to $aSlotTime=10\mu s$,  hence we have assumed the inter-arrival time of incoming data packets at each station to follow a geometric distribution  $Geom(e^{-\lambda\cdot aSlotTime})$.

%%%% UPPAAL TIME-AUTOMATON FOR SHARED MEDIUM %%%%
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[scale=0.45]{PIC/mediumTemplate}
%\caption{Template timed-automaton  of the network medium}
%\label{fig:chTA}
%\end{center}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% UPPAAL TIME-AUTOMATON FOR INPUT TRAFFIC OF A  STATION %%%%
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[scale=0.2]{PIC/trafficTemplate}
%\caption{Template timed-automaton  of the incoming traffic model}
%\label{fig:trafficTA}
%\end{center}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\subsection{Modelling with Uppaal}% and Prism}% a network of  stations based on RTS/CTS  mechanism} 
%\label{sec:modeldev}
%We have developed a DTMC model with  \prism\ representing a network of $N$ communicating stations each of which uses the 802.11 DCF RTS/CTS mechanism for transmitting data over the shared channel and according the assumptions described above. 
%The \prism\ model  for a network consisting of two stations (file \texttt{rtscts\_s2.pm}) is available for download\footnote{\url{https://sites.google.com/site/pballarini/}}, together with the Python script for generating models of  networks with an arbitrary number of stations. 
%As stated above we    started our modelling effort by developing timed automata specifications (with \uppaal), which we used as a blueprint for structuring  the   \prism\ probabilistic model. The \uppaal\ model consists of three TA templates: \texttt{Medium} (Figure~\ref{fig:chTA}), the \texttt{Channel}  (Figure~\ref{fig:stationTA}) and the \texttt{TrafficModel} (Figure~\ref{fig:trafficTA}). The  \texttt{Channel} TA encodes all phases of RTS/CTS protocol as well as the random selection of the backoff delay (in the TA corresponding with a \emph{multi-level}  non-deterministic choice of outgoing transitions for \emph{urgent locations}, i.e. \texttt{CHOOSING\_BACKOFF}. etc). Observe that the  \texttt{Channel} TA,  by interacting with other channels and with the \texttt{TrafficModel} TA, complies with both with the \emph{sender} and the \emph{receiver} behavior: while in location \texttt{WaitingForPacket2Arrive}, the arrival of a packet to be transmitted (i.e. \texttt{beginTx?} message) let the station beginning the sensing phase of the protocol, whereas the reception of an RTS packet (i.e. \texttt{emitRTS?} message) yields to the serving  (location \texttt{RECEIVE\_RTS}) of the reception request. The  \texttt{Medium} TA, respectively the  \texttt{Traffic} TA are straightforwardly from the burst-error channel model and input traffic model discussed above. Observe that in the  \texttt{Medium} and  \texttt{Traffic} automaton we abused the TA formalism by indicating probability symbols (i.e. $p$, $p1$) as transition guards: as stated above the goal for developing TA specifications   was one of guidance for encoding the actual probabilistic model within \prism.  After having simulated/debugged the TA specifications on UPPAAL we passed then to their translation into DTMC \prism\ code. 

%Here we briefly discuss the the timed automata (TA) templates  the \prism\ model is based upon.  

%Figure~\ref{fig:chTA} depicts the TA representing the network shared \texttt{channel} whereas  Figure~\ref{fig:stationTA} gives the TA representing a transmitting/receiving \texttt{station} that behaves according to the RTS/CTS mechanism. 




%\subsection{Performance analysis with Prism}
%\label{sec:prismodel}
%\paragraph{DTMC model characteristics.} The \prism\ DTMC model (see file \texttt{rtscts\_s2.pm}) consists of three main ``modules'': \texttt{globalClock}, \texttt{channel} and \texttt{station1}. Module \texttt{globalClock} represents  time elapsing  through the state variable \texttt{t} (counter of elapsed time slots) and synchronises with all time-consuming transitions (of other modules) through the labelled command \texttt{[time]}. Since \prism\ requires all state variables to be bounded (i.e. models to be finite state)  \texttt{t} is bounded by the \texttt{deadline}  parameter (Table~\ref{tab:timeparams}) and  livelock states are defined for \texttt{t=deadline}, representing the end of the model ``execution''. Module \texttt{channel} models what happens at the level of the medium and uses a number of state variables to represent the state of the medium, e.g. \texttt{nTransmit}, to count how many stations are currently occupying the channel, \texttt{transmissionType} to represent the kind of packet (RTS,CTS,DATA,ACK) currently occupying the channel, \texttt{errorBurst} to identify whether the channel is currently in a burst-error phase, etc. Channel state changes are driven by synchronisation with the \texttt{station}s modules through action labelled \texttt{[sendN]}, \texttt{[finishN]}, (\texttt{N} being the ID of the station). Finally module \texttt{station1} represents the behavior of a generic station that employs the RTS/CTS mechanism for transmitting/receiving DATA packets over the \texttt{channel}. The various phases of the protocol  (e.g. sendRTS, waitCTS, sendACK, etc) are encoded through the 29 different values of state variable \texttt{s1}. Variable \texttt{dest1} denotes the  station to to which the DATA packets are addressed, whereas a number of other variables are used to keep track of the state of  backoff procedure (\texttt{bc1},\texttt{backoff1}, \texttt{slot1}), while \texttt{incomingPacket1} indicate whether the next packet to be transmitted is already in the station buffer (such variable is ignored in saturated traffic configurations).

%\paragraph{DTMC model parameters.}  Table~\ref{tab:timeparams} resumes the values (expressed in $10\mu s$  time units) of each timing parameter of the DTMC \prism\ model.  These values comply with the IEEE 802.11 specifications~\cite{ieee80211_97} and are based on the assumption that in our DTMC model a discrete time unit  is assumed to correspond to $10\mu s$.%, hence, to comply with the IEEE 802.11 specifications~\cite{ieee80211_97} the value of $sSlotTime$ is corresponds to 2 time units.%By default a time unit of the DTMC for 802.11 DCF is assumed to coincides with the duration of $aSlotTime$, that according to the 




\noindent
Table~\ref{tab:chanerrorparams} depicts  parameters related to the  burst-error behaviour of the channel\footnote{\footnotesize The relationship between  such (\prism) parameters and the corresponding transition probability in the schematic   DTMC model  of Figure~\ref{fig:burstnoisedtmc} is indicated in between brackets next to a parameter's name.}  and parameters related to the input traffic  which are summarised in Table~\ref{tab:chanerrorparams}. 





%Parameters in Table~\ref{tab:chanerrorparams} are related to  the transition probability  of the schematic burst-error DTMC model (Figure~\ref{fig:burstnoisedtmc}) in the following manner: \texttt{mediumErrorEnterSpikeRate}=$p$, \texttt{mediumErrorExitSpikeRate}=$p'$, 

%\noindent
%Finally Table~\ref{tab:trafficparams} depicts the input traffic related parameters of \prism\  DTMC model. 

%\begin{table}[htp]
%\scriptsize
%\begin{center}
%\begin{tabular}{|c|c|c|}
%\hline
%name & meaning & definition/value \\
%\hline
%%&&\\
%\texttt{aSlotDurationInSeconds}   &  duration in sec of a time-slot & $10^{-5 }$\\
%\texttt{lambda}    & traffic arrival  rate  (Poisson) & variable \\
%\texttt{p1} &  prob. of an arrival in next time-slot  & $e^{-\texttt{lambda}\cdot\texttt{aSlotDurationInSeconds}}$\\
%\hline
%\end{tabular}
%\end{center}
%\caption{Input traffic parameters of Prism  DTMC  network model}% : first measurements}
%\label{tab:trafficparams}
%\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Reward-based measures for performance analysis of the network model.} To analyse the  performances of a network  we have equipped the \prism\ DTMC model with a number of state/transition rewards (an exert  of which is given in Table~\ref{tab:rewardsfunction}).  We have then introduced a   a number of formal properties, mainly of \emph{reward-based} nature,  written in the temporal logic specification language of \prism~\cite{prism}.   In the following we describe examples of a few  relevant properties  and present the outcome of their assessment. 




\noindent
\begin{itemize}
\item {\bf Throughput}: the number of successfully transmitted  packets per time unit. 
$$
\psi_1=\text{\texttt{R}\{``\texttt{throughput}''\}=?}[F\ t=\text{deadline}]
$$
Observe that the definition of the \texttt{throughput} reward requires the model to be capable of storing the date of the most recent successfully transmitted packet (stored in variable \texttt{lastTransmissionDate} of module \texttt{globalClock}) other than counting the number of successfully transmitted DATA packets  (stored in variable \texttt{successfulTx} of module \texttt{globalClock}). Therefore the \texttt{throughput} reward in \prism\ DTMC model is defined as follows: 

\begin{scriptsize}
$$
\texttt{throughput} = 10^5\cdot \texttt{successfulTx} / \texttt{lastTransmissionDate}
$$
\end{scriptsize}
where $10^5$ is the conversion factor to obtain a \emph{packets-per-second}  (rather than a  \emph{packets-per-timeSlot}) measure. 

%rewards "throughput"
%	[end] (lastTransmissionDate>0) : 100000*successfulTx/successfulTx;
%endrewards 


\item {\bf Busy time ratio}: the ratio between  the channel  busy time (the time the channel is occupied with some transmission)  and the total  time within reaching of model's time $deadline$.% state (i.e. the live-lock state representing the termination of the observation). 

$$
\psi_2=\text{\texttt{R}\{``busyTimeRatio ''\}=?}[F\ t=\text{deadline}]
$$
%\item {\bf Average forwarding turnaround time}: average time needed to forward a packet from a forwarding station to a target station. That is the delay  (measured in model time unit, i.e. 10$\mu$s) from the moment  the forwarding station receives the packet to the moment the packet is successfully received to the target.  \\
%send a packet, from the moment the station receives it to the moment it is successfully sent\\
%\item {\bf Average backoff round at transmission}: the average number of collisions occurred to successfully transmit a packet (from source to destination). %at a forwarding station between the moment it receives the packet and the moment the packet is successfully received by the target station.\\
\end{itemize}


\begin{figure*}
\begin{center}
%\hfill
\subfigure[Throughput]{\includegraphics[scale=.2]{PIC/throughputVnStations}\label{fig:attTX}}
%\hskip 3ex
\subfigure[BusyTimeRatio]{\includegraphics[scale=.2]{PIC/busyTimeRatioVnumStations2}}
\subfigure[saturated traffic]{\includegraphics[scale=.2]{PIC/throughputVspikeErrornStations}}
%\hskip 3ex
\subfigure[\small 2 stations, non-saturated traffic]{\includegraphics[scale=.2]{PIC/throughputVspikeErrornStations_diffLamda}}
\label{fig:BTR}
%\hfill
\caption{Impact of network dimension on non-saturated traffic}
\label{fig:impactNetDim}
\end{center}
\end{figure*}


\subsection{Mesurements}
\label{sec:measures}
We have designed experiments aimed at assessing the performances of the network model in different respects. Specifically we  have assessed the impact of: 1) a faulty channel, 2) the incoming traffic,   3) the network dimension (i.e. the number of stations in the network) and 4) the packet size on the network performances. The results presented below have been all obtained through experiments executed with \prism\ \emph{statistical engine}, with the following settings: a $99\%$ confidence level and a fixed sample size of a 1000 paths. We stress that, because of the prohibitive  complexity of the network model  (which would result in a huge space state for the corresponding DTMC), using the statistical engine of \prism\ was the only realistic option. 

\paragraph{Nominal maximum busyTimeRatio.} We observe that the busyTimeRatio (BTR) of a network whose stations use the  RTS/CTS MAC scheme is upper bounded by a \emph{nominal maximum}  which corresponds with an ideal (hypothetical) situation where a continuos flow of DATA packet are transmitted without inter-arrival delay and in absence of collisions. In such situation the BTR is given by the ratio  of  busy-time over total-time for successfully  transmitting, where the latter (in absence of collisions) is straightforwardly obtained by considering the   \texttt{DIFS}-RTS-\texttt{SIFS}-CTS-\texttt{SIFS}-DATA-\texttt{SIFS}-ACK sequence, that is: 
\begin{equation}
\label{eq:nmbtr}
NominalMaxBTR = TXtime/ (SENSEtime+TXtime)
\end{equation}
where $TXtime\!=\!RTS\!+\!CTS\!+\!DATA\!+\!ACK$, is the total transmission time and $SENSEtime\!=\!\texttt{DIFS}\!+\!3\texttt{SIFS}$ is the total carrier-sensing time. From parameters in Table~\ref{tab:timeparams}, we have that $NominalMaxBTR\!=\!80/88\!=\! 0.909$, meaning that the optimal channel utilisation for a WiFi based on RTS/CTS 802.11 MAC cannot trespass $\sim\!90\%$. In the remainder we will see that  the BTR measures obtained through \prism\ exhibit  indeed an asymptotic  profile towards $NominalMaxBTR$. 



%\paragraph{Impact of incoming traffic.} Figure~\ref{fig:exptraffic}\\

\paragraph{Impact of network dimension and incoming traffic.} Figure~\ref{fig:impactNetDim} depicts results of experiments aimed at assessing the impact of the network dimension (num. of stations) on the performance and under the ideal channel hypothesis. Specifically  Figure~\ref{fig:impactNetDim}(a) (resp. Figure~\ref{fig:impactNetDim}(b)), displays the network throughput (resp. BTR) obtained by assessing formula $\psi_1$ (resp.  $\psi_2$)  in function of the incoming traffic rate ($\lambda$) in a non-saturated network and considering  networks of different   dimensions.  As expected both the throughput and  the BTR,  exhibits an asymptotic profile (the faster the inter-arrival rate the higher the throughput, resp. the  BTR) which is upper bounded by the throughput under saturated regime (which is $\sim\! 640$ packets per second), resp. the saturated nominal maximum BTR~(\ref{eq:nmbtr}).\\

%\paragraph{Impact of packet sizel.} Figure~\ref{fig:exptraffic}\\


\noindent
Results presented in Figure~\ref{fig:impactNetDim} refer to the \emph{ideal channel} setting of the model, meaning that a packet being transmitted has virtually zero probability of being dropped because of an error affecting the channel\footnote{We used  \texttt{mediumErrorSpikeFrequency}=200, i.e. prob. the channel enters burst-error state is $p=10^{-200}$}. 

\paragraph{Impact of faulty channel.} Figure~\ref{fig:expfaultychan} illustrates results of experiments aimed at assessing the effect that a faulty channel has on the network performances.  The  network throughput measured  in function of the \texttt{mediumErrorSpikeFrequency}  parameter (i.e. in function of the  probability the channel enters a burst-error phase, see Table~\ref{tab:chanerrorparams}) is given in Figure~\ref{fig:expfaultychan}(a), showing that the throughput increases as the probability of the channel's  burst error  decreases, however it is unaffected by the network  dimension (identical plot for different number of stations) indicating that the performances gradient induced by the network dimension in case of ideal channel (Figure~\ref{fig:impactNetDim}) fades away in presence of a faulty channel. The remaining settings for these experiments are: saturated traffic, \texttt{mediumErrorSpikeLength}=3 and a 50\% chance that an error actually occurs ( \texttt{mediumErrorRateWhileSpike}=0.5) when the channel is in  burst-error phase.    


%\begin{figure*}
%\begin{center}
%%\hfill
%\subfigure[saturated traffic]{\includegraphics[scale=.25]{PIC/throughputVspikeErrornStations}}
%\hskip 3ex
%\subfigure[\small 2 stations, non-saturated traffic]{\includegraphics[scale=.25]{PIC/throughputVspikeErrornStations_diffLamda}}
%\label{fig:BTR}
%\hfill
%\caption{Impact of faulty channel on a network performances}
%\label{fig:expfaultychan}
%\end{center}
%\end{figure*}
\noindent
Conversely Figure~\ref{fig:expfaultychan}(b) shows that  the burst error probability has different effects on the throughput  a non-saturated  network of fixed dimension (i.e. 5 stations) depending of the traffic arrival rates. 

\paragraph{Other measurements.} Apart from the throughput and BTR measures we developed  a number of other performance indicators which we also assessed against  different configurations of the model. Examples of such farther measures are the {\bf Average forwarding turnaround time} (i.e. average time needed to forward a packet from a source  station to a target station), and {\bf Average backoff round at transmission} (i.e. the average number of collisions occurred to successfully transmit a packet from source to destination). For the sake of space we refrain from presenting these results here. 



==> sectionsCR/modelling_80211p.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Performance analysis of 802.11 DCF through the PRISM model checker}
%\section{Performance modelling of 802.11\lowercase{p} MAC}
\section{SSN models  of 802.11/802.11\lowercase{p} networks}
\label{sec:perfanalysis80211p}





%\subsection{Modelling assumptions}
%\paragraph{Modelling assumptions.} 


%\paragraph{Input traffic.}
%\label{sec:trafficmodel}
%To analyse the effect that different traffic conditions have on the network performances we modelled the input traffic at each station as a Poisson process with rate $\lambda\!\in\!\mathbb{R}_{\geq 0}$, hence we assumed  that the inter-arrival time of incoming data follows a negative   exponential distribution of  rate $\lambda$, i.e. $Exp(\lambda)$. However since our models are DTMC (hence time is inherently discrete)  we have adopted a geometric  approximation of the negative exponential distribution. Specifically  given that a time unit in our DTMC model of 802.11 DCF corresponds to $aSlotTime=10\mu s$,  hence we have assumed the inter-arrival time of incoming data packets at each station to follow a geometric distribution  $Geom(e^{-\lambda\cdot aSlotTime})$.




%\subsection{SSN model of 802.11p}
%\label{sec:ssnmodel80211p}
%In order to cope with the inherent complexity of the 802.11p MAC protocol we  have adopted a \emph{coloured} extension of the Generalized Stochastic Petri Nets (GSPN) formalism~\cite{ABC+95}, namely the Stochastic Symmetric  Net (SSN)~\cite{Chiola:1993:SWC:626501.626829}, to build a formal model of a network whose nodes employ EDCA scheme. SSN extends GSPN  in that tokens may be associated with a type (i.e. a  colour)  therefore allowing for  the development of much more  compact models\footnote{that can be \emph{unfolded} into an equivalent, larger, GSPN.}  than GSPN ones. 
The SSN model of the 802.11p we developed relies on the definition of a number of color classes (Table~\ref{tab:colorclasses}) and color domains (Table~\ref{tab:colordomain}) that are used to characterise the type of the various elements (places and tranisitions).  The  model consists essentially of  three parts: the \emph{802.11p core module}, representing the prioritised carrier-sensing and RTS/CTS handshaking mechanism, the \emph{backoff module}, representing the behaviour of a station in case of a collision and the \emph{medium module} representing the state of the wireless channel. For the sake of simplicity we present these 3 modules separately bearing in mind that they are part of the same SSN model. 
%representing necessary data types for the modelling of the protocol's dynamics within the SSN formalism. %Table~\ref{tab:colorclasses} and Table~\ref{tab:colordomain} depict the basic color classes, respectively the color domains used in the SSN model of 802.11p. 






\begin{figure*}
\begin{center}
%\hfill
\includegraphics[scale=.35]{PIC/80211p_RTSCTS}
\caption{SSN model of the 802.11p prioritised RTS/CTS scheme}
\label{fig:80211pRTSCTS}
\end{center}
\end{figure*}



\noindent
%\paragraph{SSN model of the RTS/CTS mechanism for 802.11p}
\paragraph{802.11p core SSN module}
Figure~\ref{fig:80211pRTSCTS} depicts the portion of the SSN model representing the traffic generation and  prioritised  RTS/CTS handshaking protocol of the stations.  It consists of three main parts: the generation of  incoming data traffic (timed transition $\mathit{PacketArrival}$), the carrier-sensing phase (timed transitions $\mathit{WaitAIFS}_i$, $\mathit{WaitSIFS}$), the packets transmission  phase (transitions $\mathit{sendRTS}$, $\mathit{sendCTS}$, $\mathit{sendDATA}$, $\mathit{sendACK}$), the handling of packets received/overheard by a station (sub-net in between places $\mathit{WaitForResponse}$, $\mathit{Receiving}$, $\mathit{ReadingPacket}$). Let's describe the various parts of the model. Place $\mathit{Idle}$ (color domain $\mathit{SP}$) is initially filled up with tokens corresponding with all pairs from $\mathit{St}\!\times\!\mathit{Pr}$, representing that each station may generate incoming traffic with any level of priority. The firing of the outgoing timed (exponentially distributed) transition $\mathit{PacketArrival}$ consumes a $\langle sa,p\rangle$ token and produces the $\langle sa,sb,p,rts\rangle$   token (added to place $\mathit{Sense}$) indicating that station $sa$ is ready to send an $rts$ request with priority $p$ to station $sb$ ($sa\!\neq\! sb$). A token $\langle sa,sb,p,pt\rangle$   in place  $\mathit{Sense}$ (representing an ongoing transmission of a packet of type $pt$ and priority $p$ from station $sa$ to $sb$) is then moved either to i) place $\mathit{Vulnerable}$ through either one of the four mutually-exclusive timed (deterministic) transition  $\mathit{WaitAIFS}_i$ (only that corresponding to the actual priority value $p$ is enabled), if  packet type $pt\!=\!rts$ and the medium remains free for  $\mathit{AIFS}_i$ time units, or through $\mathit{WaitSIFS}$ if packet type $pt\!\neq\! rts$ and medium stay free for $\mathit{SIFS}$, or if the medium gets occupied in the meantime ii) to $\mathit{GoingToBackoff}$  (through immediate transition $\mathit{SenderSenseCollision}$) if $sa$ is the sender of an $rts$ or $data$ packet or  iii) to $\mathit{WaitForResponse}$ (through immediate transition $\mathit{ReceiverSenseCollision}$) if $sa$ is a station responding with either a $cts$ or $ack$ to $sb$. A token $\langle sa,sb,p,pt\rangle$ from place $\mathit{Vulnerable}$ moves to $\mathit{Sending}$ (after $\mathit{Vuln}$ time units through timed  transition $\mathit{BeingSending}$), and in so doing it adds one (uncoloured) token to $\mathit{Medium}$ indicating that the number of transmitting stations has   increased. Observe that the immediate transition $\mathit{InternalCollision}$ (which is also consuming tokens from $\mathit{Vulnearble}$) deals with the case of   competing packets sent,  with different level of priorities,  by a common station $sa$: %to potentially different destinations $sb$ and $sc$: 
in this case  only the packet with the highest priority stays in $\mathit{Vulnerable}$, while packets with lower priority are  moved to   $\mathit{GoingToBackoff}$ (i.e. highest priority packet wins the internal competition by ``overtaking'' lower priority packets). From place $\mathit{Sending}$ a token  $\langle sa,sb,p,pt\rangle$ moves to   $\mathit{PacketSent}$ if the packet type is either $rts$, $cts$ or $data$, after a  delay corresponding with the kind of packets, and then, with no delay, it is further moved to $\mathit{WaitForResponse}$ through immediate transition $\mathit{BeginWaitingForResponse}$ which while removing a token from $\mathit{Medium}$ (hence decreasing the occupation of the wireless channel) and storing the $\langle sa,sb,p,pt\rangle$  in place $\mathit{SentPacket}$ for later retrieval, also updates the packet type of token  $\langle sa,sb,p,pt\rangle$ to $\langle sa,sb,p,pt\!+\!+\rangle$, indicating that station $sa$ is now ready to wait for a reply message (of type $pt\!+\!+$, i.e. $cts$ in reply to $rts$ or $ack$ in replay to $data$) from $sb$. 
Place $\mathit{WaitForResponse}$ is initialised with marking $\langle St,s1,pr1,rts\rangle$ indicating that each station of $St$ is, initially, ready to get engaged into replying to an $rts$ request ($s1$ and $pr1$ being irrelevant at this stage). As the medium gets occupied but not garbled all tokens in $\mathit{WaitForResponse}$ are moved (with no delay) to $\mathit{Receiving}$ and from there, as soon as the channel gets free (and assuming it hasn't been garbled before) they  move on to $\mathit{ReadingPacket}$. Thus, at the end of a transmission phase, place  $\mathit{ReadingPacket}$ contains all tokens representing all possible combinations of responses that all stations may be engaged in. On completion of the transmission corresponding to token  $\langle sb,sa,p,pt\rangle$ being added to $\mathit{SentPacket}$ the corresponding token $\langle sa,sb,p_2,pt\rangle$, if present,  is consumed from $\mathit{ReadingPacket}$ (through either one of the prioritised transitions $\mathit{CorrectPacketButAck}$ or $\mathit{CorrectPacketAck}$) representing the creation of the response, by the destination station $sa$, to  the transmitted packet $pt$. 
Notice that $\mathit{CorrectPacketButAck}$  triggers the response to an $\mathit{rts}$, $\mathit{cts}$ or $\mathit{data}$  packet   by adding the token $\langle sa,sb,p,pt\!+\!+\rangle$ to $\mathit{Sense}$ hence moving to the next step of the RTS/CTS protocol for the processed packet. Conversely $\mathit{CorrectPacketAck}$ represents the end of the RTS/CTS handshaking hence it puts back a $\langle sa,p\rangle$ token to $\mathit{Idle}$ which restart  the cycle for the transmission of a priority level $p$ packet by station $sa$.  On the other hand all  tokens $\langle sa,sb,p,pt\rangle$ that remain in $\mathit{ReadingPacket}$ after a response to the transmitted packet has been treated (through either $\mathit{CorrectPacketButAck}$ or $\mathit{CorrectPacketAck}$)   are either put back to $\mathit{WaitForResponse}$ (if they represent a receiver, i.e. transition $\mathit{ReceiverWrongPacket}$) or  they are moved to $\mathit{GoingToBackoff}$ (if they represent a sender that  was expecting either a   $\mathit{cts}$ or an $\mathit{ack}$ response to a previosuly sent packet $\mathit{rts}$ or $\mathit{data}$). 
%whereas it moves to $\mathit{WaitForResponse}$ if packet type is $ack$. 


\begin{figure*}
\begin{center}
%\hfill
\includegraphics[scale=.35]{PIC/80211p_backoff}
\caption{SSN model of the 802.11p backoff mechanism}
\label{fig:80211pbackoff}
\end{center}
\end{figure*}

\noindent
%\paragraph{SSN model of the RTS/CTS mechanism for 802.11p}
\paragraph{802.11p backoff SSN module}
With the 802.11p DCF the selection of the \emph{backoff} duration, i.e. the selection of the number of  \emph{time slots} a packet has to wait before starting a new transmission attempt, depends on the priority class of the packet as well as on the backoff round, i.e. the number of times a packet has unsuccessfully went through the carrier-sensing phase without winning the contention. Therefore a model of 802.11p backoff procedure must be equipped with necessary  means to take  into account the priority level of each packet hence  the size of the contention window for each  priority level.
Figure~\ref{fig:80211pbackoff} depicts the SSN subnet   dedicated to modelling of the randomised selection of the backoff delay for a packet of a given priority level $p$. A backoff begins when a token $\langle sa,sb,p\rangle$ is added to place $\mathit{GoingToBackoff}$ (color domain $\mathit{BP}$) indicating that something went wrong (e.g. a collision or a lack of handshaking) during the transmission of  a priority $\mathit{p}$ packet from station $\mathit{sa}$ towards $\mathit{sb}$. The first step then is the updating of the backoff round counter  which boils down to adding of a token $\langle sa,sb,p,tx \rangle$  to place $\mathit{TxAttemptsCounter}$ (whose  color domain is $\mathit{SRPCoun}t$ and where  variable $\mathit{tx}\!\in\! \mathit{TxCount}$ stores the backoff counter)  through either   transition $\mathit{GoToBackoff}$ (enabled if the failed transmission attempt is the first one, hence initialising $\mathit{tx}$ to color $\mathit{tx_1}$)  or through transition $\mathit{ReturnToBackoff}$ (enabled by any further failed transmission attempt and increasing $\mathit{tx}$ by 1). 
Once a token  $\langle sa,sb,p \rangle$ enters place $\mathit{ChoosingBackoff}$ having, in the process, also added (or updated) a  $\langle sa,sb,p,tx \rangle$  token to  place $\mathit{TxAttemptsCounter}$, either one between the  mutually exclusive transitions $\mathit{ChooseBackoff}$ or $\mathit{DropPacket}$ transition is enabled. Transition $\mathit{ChooseBackoff}$ realises the probabilistic selection of the backoff counter value $b$, corresponding to the priority level $p$ of the \emph{backoffing} packet, by adding token $\langle sa,sb,p,b\rangle$ to place $\mathit{BackoffCounter}$. Such a  selection is achieved through  randomly choosing (through  the test arc between  transition $\mathit{ChooseBackoff}$ and place $\mathit{BackoffMappings}$) a token   $\langle p,tx,b \rangle$ among those specified by the invariant marking  of  $\mathit{BackoffMappings}$ given  in Table~\ref{tab:marking}. 


\begin{figure}
\begin{center}
%\hfill
\includegraphics[scale=.35]{PIC/80211p_medium}
\caption{SSN model of the shared medium}
\label{fig:80211pmedium}
\end{center}
\end{figure}



%Figure~\ref{fig:backoffmapssn} depicts the SSN subnet   dedicated to modelling of the randomised selection of the backoff delay for a packet of a given priority level $p$. Place $\mathit{GointToBackoff}$ (color domain $BP$) is devoted to contain tokens $\langle sa,sb,p \rangle\in St\times St\times Pr$ that represent  a failed transmission attempt of a priority $p$ packet   from a source station $sa$ to a destination station $sb$. A token  $\langle sa,sb,p \rangle$ in place place $\mathit{GointToBackoff}$ moves to place $\mathit{ChoosingBackoff}$ either through transition $\mathit{GoToBackoff}$, if the failed transmission attempt is the first one, or through  transition \texttt{ReturnToBackoff} if $\langle sa,sb,p \rangle$ represents a further failed transmission attempt. 

%Counting of successive transmission attempts is kept track of  by tokens $\langle sa,sb,p,tx \rangle$  of place $\mathit{TxAttemptsCounter}$ (color domain $\mathit{SRPCoun}t$) and specifically by  variable $\mathit{tx}\!\in\! \mathit{TxCount}$ ($\mathit{TxCount}$ being an ordered class),  is set to color $tx_1$, in case of the first backoff round (i.e. through transition \texttt{GointToBackoff}), or incremented, in case of a further backoff attempt (i.e. \texttt{ReturnedToBackoff}). Once a token  $\langle sa,sb,p \rangle$ enters place \texttt{ChoosingBackoff} having, in the process, also added (or updated) a token $\langle sa,sb,p,tx \rangle$  to  place \texttt{TxAttemptsCounter}, either one between the  mutually exclusive transitions $\mathit{ChooseBackoff}$ or $\mathit{DropPacket}$ transition is enabled. Transition $\mathit{ChooseBackoff}$ realises the probabilistic selection of the backoff counter value $b$ corresponding to the priority level $p$ of the \emph{backoffing} packet. Such a randomised selection is achieved through   the test arc between  transition $\mathit{ChooseBackoff}$ and place $\mathit{BackoffMappings}$ (color domain $\mathit{BPMap}$) which allows for selecting  a random token $\langle p,tx,b \rangle$ among those of the initial (and invariant) marking $\mathit{BM}_0$ of  $\mathit{BackoffMappings}$. 

The marking of $\mathit{BackoffMappings}$ associates with each priority level $\mathit{pr_i}$ and re-transmission attempt $\mathit{tx_j}$ the corresponding CW expressed as  the union of color subclasses $\cup_{k=1}^{k'} bs_k$ (where $k'$ is a function of $pr_i$ and $tx_j$). 
Therefore, for example,  for the first re-transmission attempt (i.e. $\mathit{tx=tx_1}$) of a priority  $p_1$ packet  the backoff value $b$ is chosen randomly as $b\in\ \mathit{bs_1}=\mathit{\{b1,\ldots ,b4\}}$ (which corresponds with the narrowest CW for the AC\_V0 priority category) as the initial marking $\mathit{BM_0}$ contains  tokens $<pr1,tx1,bs1>$.  Similarly for the second re-transmission attempt (of a priority  $p_1$ packet) $b$ is chosen randomly as $b\in\ \mathit{bs_1}\cup \mathit{bs_2}=\mathit{\{b1,\ldots ,b8\}}$ as marking $\mathit{BM_0}$ contains  tokens $<pr1,tx2,bs1+bs2>$ and so on.  Once a $\langle sa,sb,p,b\rangle$ token is added to place $\mathit{BackoffCounter}$ (i.e. the backoff delay $b$ is selected) the actual backoff (sensing) period  begins: $b$ is decremented every $\mathit{aSlot}$ time units (deterministic transition $\mathit{DecrementBackoff}$) however, as soon as the medium gets occupied, the decrement of $b$ is suspended by moving token $\langle sa,sb,p,b\rangle$ from  $\mathit{BackoffCounter}$ to $\mathit{PausingBackoff}$ (immediate transition $\mathit{PauseBackoff}$).  Token $\langle sa,sb,p,b\rangle$ is moved back to  $\mathit{BackoffCounter}$ only after the channel got freed and stayed free for $\mathit{AIFS_i}$ time units (where $i\!\in\!\{1,2,3,4\}$ denotes the priority level $p$  of the  backoff-ing packet). The backoff  for a token $\langle sa,sb,p,b\rangle$ ends as soon as the backoff counter has reached 1 (i.e. $b\!=\!b1$): at this point token $\langle sa,sb,p,b1\rangle$ is removed from $\mathit{BackoffCounter}$ (immediate transition $\mathit{ExitBackoff}$) and $\langle sa,sb,p,rts\rangle$ is pushed back to $\mathit{Sense}$ which represent the re-start of the transmission procedure for station $\mathit{sa}$ to sent a priority $p$ packet to $\mathit{sb}$.



\noindent
%\paragraph{SSN model of the RTS/CTS mechanism for 802.11p}
\paragraph{802.11p medium SSN module}
Figure~\ref{fig:80211pmedium} shows the part of the SSN model  representing the shared channel. It consists of 2 uncoloured places: $\mathit{Medium}$,   whose marking corresponds with the number of transmitting stations, and  $\mathit{Garbled}$,  which contains a token whenever a collision has taken place or an error spike has occurred on the channel.  Transition $\mathit{GettingGarbled}$ sets the state of the medium to \emph{garbled} (adding a token in place $\mathit{Garbled}$) as soon as  $\mathit{Medium}$ contains at least 2 tokens (i.e. at least two stations are transmitting).   Transition $\mathit{EndingGarbled}$ ends the \emph{garbled} state of the medium by removing a token from $\mathit{Garbled}$ as soon as the $\mathit{Medium}$ is emptied.  Place $\mathit{SentPacket}$ (domain $P$) stores the information relative to an ongoing transmission in terms of   a token $\mathit{\langle sa,sb,p,pt\rangle}$ where  $sa$ is the sender station, $sb$ the receiver ,$p$  the priority level $p$ and  $tp$ the packet type).



\subsection{Performance analysis with Cosmos}
\label{sec:cosmosmodel}
\paragraph{Stochastic symmetric Nets model.}

\paragraph{SSN model parameters.}  



%\subsection{Mesurements}
%\label{sec:measures80211p}


%\paragraph{Impact of incoming traffic.} Figure~\ref{fig:exptraffic}\\


==> sectionsCR/preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}
%The performance analysis study we present in the remainder of the paper is based on discrete-time Markov chain models  
We briefly recall the basic notions of probabilistic model checking for discrete-time Markov chain models~\cite{KNP07a}, i.e. the  modelling framework we used in this study. %for performance analysis of the 802.11 DCF RTS/CTS mechanism. 


\begin{definition}
\label{def:dtmc}
For $AP$ a set of atomic propositions,  a labeled  discrete-time Markov chain is defined as a tuple $(S,s_0,\mathbf{P},L)$ where:
\begin{itemize}
\item $S$ is a countable set of states
\item $s_0$ is the initial state
\item $\mathbf{P}: S\times S\to[0,1]$ is the  \emph{transition probability matrix}, with   $\sum_{s'\in S} \mathbf{P}(s,s') =1$, $\forall s\in S$.
\item $L:S\to AP$ is the state labelling function assigning each state $s\in\! S$ a label of $L(s)\!\in\! AP$.
\end{itemize}
\end{definition}
Time in DTMCs is inherently discrete and each transition is assumed to consume exactly one unit of time. 
Therefore for any two states $s,s'\in S$, $\mathbf{P}(s,s')$ denotes the probability of a transition from $s$ to $s'$ to occur during one   time unit. 
Generally the set of states is a subset of the $n$-dimensional real space (i.e. $S\subseteq \mathbb{R}^n$), whereas the atomic propositions of $AP$ are symbolic names corresponding to boolean propositions built on top of the state variables characterising $S$ (e.g. $channelBusy\!\in\! AP$, with $channelBusy\equiv (nTrasmit\!>\!0)$, where $nTransmit$ is a state variable counting the number transmitting stations at a given moment in time). 
Events of a DTMC can be assimilated with \emph{execution paths}, i.e.   (infinite) sequences of states  $\omega\!=\! \omega(0), \omega(1), \dots$ with $\omega(i)\!\in\! S$, $\forall i$.  It is straightforward to see that the transition matrix $\mathbf{P}$ induces a probability measure on the space of infinite paths sharing a common finite-prefix (i.e. \emph{cylinder set}), therefore the probability of DTMC events (i.e. occurrence of set of paths with common finite prefix) is well defined~\cite{KNP07a}. 

The probabilistic computational tree logic (PCTL~\cite{HansJons89}), i.e. the extension of CTL~\cite{Clarke86} to probabilistic models, is a specification language for characterising events of a DTMC. 
 Below we recall its ``standard''  syntax together with the extended syntax for stating \emph{reward-based} properties (supported by the \prism\ tool).

\begin{definition} The syntax of the PCTL logic is defined as follows
\label{def:pctl}
\begin{equation}
\begin{aligned}
\phi &:= a\mid tt \mid\lnot\phi\mid\ \phi \land\phi \mid {\mathcal P}_{\sim p}(\varphi) \\%&\text{(state-formulae)}\\
\varphi &:= X^{\leq k}\ \phi\mid  \phi\ U^{\leq k}\phi %&\text{(path-formulae)}
\end{aligned}
\end{equation}
where $a\!\in\! AP$, $\sim \in\!\{<,\leq,\geq,>,=\}$, $p\!\in\! [0,1]$ $k\!\in\! \mathbb{N}$, $X$ is the \emph{neXt} operator, $U$ is the \emph{Until} operator, $\phi$ denotes a state-formula.  %$q\!\in\! \{=\!?\}\cup (\{<,\leq,\geq,>,=\}\times [0,1])$
\end{definition}


For the sake of brevity we only informally describe the semantics of PCTL formulae, referring the reader to the literature~\cite{HansJons89,KNP07a} for a formal treatment. 
Assessing  of PCTL ``probabilistic'' state formulae $ {\mathcal P}_{\sim p}(\varphi) $ requires evaluating  the probability  measure of   paths satisfying  $\varphi$, which in turns requires identifying paths that validate $\varphi$. As an example of a typical \emph{Until} formula let's consider  $\varphi\equiv (nTrasmit\!\leq\!1) U^{\leq 100} (nbSuccRecPackets=2)$ which is verified by all paths corresponding to successful reception (within $k=100$ time units) of two data packet ($nbSuccRecPackets=2$) in absence of collisions (i.e. never  the channel has been occupied by more than a station, i.e. $\varphi\equiv (nTrasmit\!\leq\!1)$). 
Observe that apart from   \emph{qualitative} formulae, i.e. formulae which evaluate to a boolean value as given in~(\ref{def:pctl}), \prism\ also supports \emph{quantitative} formulae, i.e. formulae which evaluate to a real value,  through the following syntax ${\mathcal P}_{= ?}(\varphi)$ (i.e. the value being the probability measures of paths verifying $\varphi$). 
% PCTL path formulae are evaluated against DTMC paths, thus,  for example,  formula $\varphi\equiv (nTrasmit\!\leq\!1) U^{\leq 100} (nbSuccRecPackets=2)$ is verified by all paths corresponding to successful reception (within $k=100$ time units) of two data packet ($nbSuccRecPackets=2$) in absence of collisions (i.e. never  the channel has been occupied by more than a station, i.e. $\varphi\equiv (nTrasmit\!\leq\!1)$). 
%The verification of PCTL ``probabilistic'' state formulae $ {\mathcal P}_{\sim p}(\varphi) $ is achieved by comparison of the probability  measure of  all paths satisfying $\varphi$ against threshold $\sim p$


To improve the performance evaluation capabilities a DTMC ${\mathcal D}=(S,s_0,\mathbf{P},L)$ may be enriched with several    reward structures, where a reward structure is  either a state-reward function  $\underline{\rho}:S\to\mathbb{R}_{\geq 0}$ or a transition-reward function  $\iota:S\!\times\! S\to \mathbb{R}_{\geq 0}$  assigning non-negative real-valued rewards to states, resp. transitions, of ${\mathcal D}$.  \prism\  allows for enriching DTMC models with  several reward structures  and supports  an extension of  standard PCTL syntax, featuring  the following reward-based operators:


\begin{definition} The syntax  of \prism-supported  PCTL  reward-based properties  is defined as follows
\label{def:pctlrewards}
\begin{equation}
\begin{aligned}
\psi &:= \texttt{R}[''\rho'']_{\sim r}(\texttt{C}^{\leq k}) \mid \texttt{R}[''\rho'']_{\sim r}(\texttt{I}^{= k}) \mid \texttt{R}[''\rho'']_{\sim r}(\texttt{F} \phi) \\%&\text{(state-formulae)}\\
\end{aligned}
\end{equation}
where  $\sim \in\!\{<,\leq,\geq,>,=\}$, $r\!\in\! \mathbb{R}_{\geq 0}$, $k\!\in\! \mathbb{N}$, $\rho$ is either a state or a transition reward function,  $\phi$ is a PCTL state-formula.
\end{definition}

\noindent
Informally the semantics of \prism-supported reward-based formulae is as follows: $\texttt{R}[''\rho'']_{\sim r}(\texttt{C}^{\leq k}) $ (resp. $\texttt{R}[''\rho'']_{\sim r}(\texttt{I}^{= k}) $) refers to the average value of reward $\rho$ cumulated up to (resp. computed exactly at)  time $k$ whereas $\texttt{R}[''\rho'']_{\sim r}(\texttt{F} \phi)$ refers to the average value of $\rho$ up to reaching a $\phi$-state (i.e. a state that satisfies $\phi$). 
As for standard PCTL \prism\ support both a \emph{qualitative} and \emph{quantitative} semantics for reward formulae, where the quantitative  semantics is associated with the syntax  $\texttt{R}[''\rho'']_{= ?}(\texttt{C}^{\leq k}) $. 
For the formal definition of the semantics of \prism-supported reward-based formulae we refer to~\cite{KNP07a}. 

